The Young, Massive, Star Cluster Sandage-96 After the Explosion of SN 2004dj in NGC 2403

The bright Type II-plateau supernova (SN) 2004dj occurred within the young, massive stellar cluster Sandage-96 in a spiral arm of NGC 2403. New multi-wavelength observations obtained with several ground-based and space-based telescopes are combined to study the radiation from Sandage-96 after SN 2004dj faded away. Sandage-96 started to dominate the flux in the optical bands starting September 2006 (~800 d after explosion). The optical fluxes are equal to the pre-explosion ones within the observational uncertainties. An optical Keck spectrum obtained ~900 d after explosion shows the dominant blue continuum from the cluster stars shortward of 6000 \AA as well as strong SN nebular emission lines redward. The integrated spectral energy distribution (SED) of the cluster has been extended into the ultraviolet region by archival XMM-Newton and new Swift observations, and compared with theoretical models. The outer parts of the cluster have been resolved by the Hubble Space Telescope, allowing the construction of a color-magnitude diagram. The fitting of the cluster SED with theoretical isochrones results in cluster ages between 10--40 Myr, depending on metallicity and the model family. The isochrone fitting indicates that the resolved part of the cluster has a bimodal age distribution: a younger population at ~10--16 Myr, and an older one at ~32--100 Myr which is similar to the age distribution of the nearby field stars. These stars may have been captured from the field during the cluster formation. The young age of Sandage-96 suggest 12 < M_prog < 20 M_\odot as the most probable mass range for the progenitor of SN 2004dj. This is consistent with, but perhaps slightly higher than, most of the other Type II-plateau SN progenitor masses determined so far.

==> abstract <==
The bright Type II-plateau supernova (SN) 2004dj occurred within the
young, massive stellar cluster Sandage-96 in a spiral arm of NGC~2403.
New multi-wavelength observations obtained with several ground-based
and space-based telescopes are combined to study the radiation from
Sandage-96 after SN~2004dj faded away.  Sandage-96 started to dominate
the flux in the optical bands starting September 2006 (~800 d
after explosion). The optical fluxes are equal to the pre-explosion
ones within the observational uncertainties. An optical Keck spectrum
obtained ~900 d after explosion shows the dominant blue continuum
from the cluster stars shortward of 6000 \AA as well as strong SN
nebular emission lines redward.  The integrated spectral energy
distribution (SED) of the cluster has been extended into the
ultraviolet region by archival XMM-Newton and new Swift
observations, and compared with theoretical models. The outer parts of
the cluster have been resolved by the Hubble Space Telescope,
allowing the construction of a color-magnitude diagram. The fitting of
the cluster SED with theoretical isochrones results in cluster ages
distributed between 10 and 40 Myr, depending on the assumed
metallicity and the theoretical model family.  The isochrone fitting
of the color-magnitude diagrams indicates that the resolved part of
the cluster consists of stars having a bimodal age distribution: a
younger population at ~10--16 Myr, and an older one at
~32--100 Myr.  The older population has an age distribution
similar to that of the other nearby field stars.  This may be
explained with the hypothesis that the outskirts of Sandage-96 are
contaminated by stars captured from the field during cluster
formation.  The young age of Sandage-96 and the comparison of its pre-
and post-explosion SEDs suggest 12 < M_prog < 20 M_\odot
as the most probable mass range for the progenitor of
SN~2004dj.  This is consistent with, but perhaps slightly higher than,
most of the other Type II-plateau SN progenitor masses determined so
far.
